Single-domain Bose condensate magnetometer achieves energy resolution per bandwidth below $\hbar$

We present a magnetic sensor with energy resolution per bandwidth $E_R < \hbar$. We show how a $^{87}\mathrm{Rb}$ single domain spinor Bose-Einstein condensate, detected by non-destructive Faraday-rotation probing, achieves single shot dc magnetic sensitivity of $72(8)~\mathrm{fT}$ measuring a volume $V= 1091(30)~\mu\mathrm{m}^3$ for $3.5~\mathrm{s}$, and thus $E_R = 0.075(16)~\hbar$. We measure experimentally the condensate volume, spin coherence time, and readout noise, and use phase-space methods, backed by 3+1D mean-field simulations, to compute the spin noise. Contributions to the spin noise include one-body and three-body losses and shearing of the projection noise distribution, due to competition of ferromagnetic contact interactions and quadratic Zeeman shifts. Nonetheless, the fully-coherent nature of the single-domain, ultracold two-body interactions allows the system to escape the coherence vs.~density trade-off that imposes an energy resolution limit on traditional spin-precession sensors. We predict that other Bose-condensed alkalis, especially the antiferromagnetic $^{23}\mathrm{Na}$, can further improve the energy resolution of this method.

==> NewCommands.tex <==
\definecolor{mygreen}{rgb}{0,0.5,0} 
\definecolor{mygrey}{rgb}{0.5,0.5,0.5} 
\definecolor{myred}{rgb}{0.75,0,0} 
\definecolor{myblue}{rgb}{0,0,0.75} 
\definecolor{mymagenta}{cmyk}{0,1,0,0.12} 
\definecolor{mycyan}{cmyk}{1,0,0,0.12} 
\definecolor{myorange}{rgb}{1,0.5,0} 
\definecolor{myviolet}{rgb}{0.5,0.0,0.75} 

\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bd}{{\bf d}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bq}{{\bf q}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bx}{{\bf x}}
%\newcommand{\br}{{\bf r}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bv}{{\bf v}}
\newcommand{\brho}{{\bf \rho}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}


\newcommand{\btext}[1]{{\color{myblue}#1}}
\newcommand{\newbtext}[1]{{\color{myblue}#1}}
\renewcommand{\newbtext}[1]{#1}
\newcommand{\gtext}[1]{{\color{mygreen}#1}}
\newcommand{\otext}[1]{{\color{myorange}#1}}
\newcommand{\vtext}[1]{{\color{myviolet}#1}}
\newcommand{\mtext}[1]{{\color{magenta}#1}}
\newcommand{\ctext}[1]{{\color{cyan}#1}}
\newcommand{\rtext}[1]{{\color{myred}#1}}
\newcommand{\stext}[1]{{\color{myred}\sout{#1}}}
%\renewcommand{\btext}[1]{#1}
\renewcommand{\stext}[1]{}

\newcommand{\var}{{\rm var}}
\newcommand{\cov}{{\rm cov}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\rb}{\ensuremath{ ^{87}\mathrm{Rb} } }
\newcommand{\mean}[1]{\langle #1 \rangle}

 \newcommand{\Tone}{\ensuremath{{T}_1} }
\newcommand{\Ttwo}{\ensuremath{{T}_2} }
 \newcommand{\Tevol}{\ensuremath{T_{\rm evol}}}
  \newcommand{\Tcycle}{\ensuremath{T_{\rm cycle}}}
 \newcommand{\Tseq}{\ensuremath{T_{\rm seq}}}
\newcommand{\PRLsection}[1]{\noindent {\it#1} -}
\newcommand{\arctantwo}{{\rm arctan2}}

\newcommand{\supin}{^{({\rm in})}}
\newcommand{\supout}{^{({\rm out})}}

\newcommand{\NA}{N}
\newcommand{\NL}{N_{\rm L}}
\newcommand{\vx}{\ensuremath{\vec{x}}}
\newcommand{\vy}{\ensuremath{\vec{y}}}
\newcommand{\vz}{\ensuremath{\vec{z}}}
\newcommand{\opf}[1]{\hat{f}_{#1}}
\newcommand{\opj}[1]{\hat{j}_{#1}}


\newcommand{\Ekin}{E_{\rm kin}}
\newcommand{\Econt}[1]{E_{\rm #1}}
\newcommand{\Eqz}{E_{\rm QZ}}
% \newcommand{\spinor}[1]{\left( #1 \right)^T }
% \newcommand{\Ttot}{T_{\rm acq}}
% \newcommand{\NA}{N_{\rm A}}
% \newcommand{\NL}{N_{\rm P}}
% 
% 
% \newcommand{\opf}[1]{\ensuremath{\hat{f}_{#1}}}
% \newcommand{\opF}[1]{\ensuremath{\hat{F}_{#1}}}
% \newcommand{\opj}[1]{\ensuremath{\hat{\jmath}_{#1}}}
% \renewcommand{\opf}[1]{\ensuremath{{f}_{#1}}}
% \renewcommand{\opF}[1]{\ensuremath{{F}_{#1}}}
% \renewcommand{\opj}[1]{\ensuremath{{j}_{#1}}}




\newcommand{\circled}[1]{\textcircled{\raisebox{0.25pt}{\fontsize{6}{7}\selectfont\hspace{-2.5pt} #1}}}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\res}{\sigma}           
\newcommand{\rTF}{r_{\rm TF}}


\newcommand{\del}[1]{\rtext{\sout{#1}}}

\newcommand{\mcite}[1]{\cite{#1}}
\newcommand{\pcite}[1]{\cite{#1}.}
\newcommand{\ccite}[1]{\cite{#1},}

\newcommand{\mciteSI}[1]{~\citeSI{#1}}
\newcommand{\pciteSI}[1]{~\citeSI{#1}.}
\newcommand{\cciteSI}[1]{~\citeSI{#1},}

%FROM TEXT



\newcommand{\mysec}[1]{\noindent {{\textbf{#1}\\}}}
\renewcommand{\PRLsection}[1]{\vtext{#1}}
\newcommand{\Trelax}{T_{\rm scat}}
\newcommand{\tProbe}{\tau}
%\renewcommand{\gtext}[1]{}
\definecolor{violet}{rgb}{.5,0,.5}
\renewcommand{\vtext}[1]{{\color{violet}#1}}
\renewcommand{\mtext}[1]{{\color{magenta}#1}}
\renewcommand{\var}[1]{\ensuremath{\langle #1 ^2\rangle}}
\newcommand{\sdsbec}{SDSBEC}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\supc}{^{(\rm c)}}
\renewcommand{\supc}{^{c}}
 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\rate}[1]{\Gamma _#1}

 \newcommand{\Fpar}{F_\parallel}
 \newcommand{\Fperp}{F_\perp}
 \newcommand{\Ftheta}{F_\theta}
 \newcommand{\varFtheta}{\ensuremath{\langle \delta \Ftheta^2\rangle} }

\newcommand{\RC}{\eta}
\newcommand{\DensInt}[1]{I_{#1}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bK}{{\bf K}}
\renewcommand{\Tevol}{T}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%new ones for Science
%\newcommand{\autoref}[1]{#1}
\renewcommand{\mysec}[1]{\paragraph*{#1}}

